Challenges in Adapting ECH in TLS for Privacy Enhancement over the Internet

Security and Privacy are crucial in modern Internet services. Transport Layer Security (TLS) has largely addressed the issue of security. However, information about the type of service being accessed goes in plain-text in the initial handshakes of vanilla TLS, thus potentially revealing the activity of users and compromising privacy. The ``Encrypted ClientHello'' or ECH overcomes this issue by extending TLS 1.3 where all of the information that can potentially reveal the service type is masked, thus addressing the privacy issues in TLS 1.3. However, we notice that Internet services tend to use different versions of TLS for application data (primary connection/channel) and supporting data (side channels) such as scheduling information \textit{etc.}. %, during the active session. Although many internet services have migrated to TLS 1.3, we notice that it is only true for the primary connections which do benefit from TLS 1.3, while the side-channels continue to use lower version of TLS (e.g., 1.2) %which do not support ECH and continue to leak type of service accessed. We demonstrate that privacy information leaked from the side-channels can be used to affect the performance on the primary channels, like blocking or throttling specific service on the internet. Our work demonstrates that adapting ECH on primary channels alone is not sufficient to prevent the privacy leaks and attacks on primary channels. Further, we demonstrate that it is necessary for all of the associated side-channels also to migrate to TLS 1.3 and adapt ECH extension in order to offer complete privacy preservatio

==> tls13_sc.tex <==
Even though TLS 1.3 provides the more secure TLS handshake message exchange through parameter-wise encryption, we identified the following prominent drawbacks that deter the complete adoptions of TLS 1.3. These shortcomings impede the full scale commercial implementation of TLS 1.3 including encrypting server host identity. 

\begin{itemize}
    \item {\bf Multiple parameter-wise encryption:}
As described above, TLS 1.3 had added provisions to encrypt individual extensions of handshake messages such as security certificates. Additional encryption tends to undermine the benefits gained through latency reduction techniques such as $pre\_share\_key$. This performance erosion makes its performance equivalent to previous versions and sometimes slower for low latency applications \cite{tls13_encry_perf}. It is acting as one of deterring factors for the adoption of TLS 1.3. This could be primary reason behind secure channels other than carrying actual streaming data established by many streaming services use TLS 1.2. These are short-lived low-data secure channels. We verified this fact for Amazon prime video service.  

\item{\bf Required companion technology (DNS-over-HTTPS)}
The TLS 1.3 needed DNS-over-HTTPS technology as a pre-requisite for securely exchanging predefined security keys (i.e., $pre\_key\_share$ parameter in the ``ClientHello" handshake message). However, not all public DNS and enterprise DNSes support DNS-over-HTTPS. The primary reason is the inability of ISPs to perform tasks such as firewall protection, parental control, DNS cache management, and, importantly, malware detection. In such cases, the use of third-party DNS is also a concern for ISPs. It is evident from the concerns raised by UK ISPs and Mozilla's decision not to enable DoH by default in Firefox for UK citizens \cite{doh_isp_concern}. Even though recent works such as \cite{doh_identify} propose schemes to identify DoH traffic with high accuracy, the requirement of aligning third-party DNS policies with regional ISP policies as prescribed by regulators is challenging. Moreover, the mechanism for discovering DoH resolver within ISP is still in proposal state \cite{adpt_doh_doscover}. Standardizing these proposals will go a long way in encouraging ISPs to deploy their own DoH/DoT resolvers.

%\item{\bf ESNI issues}
%A standardization body acknowledges the need for encrypted SNI (E-SNI) with the related issues and requirements well documented in the internet-draft \cite{draft-ietf-tls-sni-encryption-09}. It categorizes various E-SNI requirements as attack prevention, fronting server-related, and other security considerations. The E-SNI is still not available as an Internet standard, but the internet-draft in an experimental version is available \cite{draft-ietf-tls-esni-13} that proposes to encrypt the entire ``clientHello" message. A slightly different version of it is already implemented and commercialized by ``Cloudflare" \cite{cf_esni} that encrypts only the SNI portion of the ``clientHello" message. It uses the Diffie-Hellman key exchange algorithm to generate a shared encryption key over an untrusted channel. This method's main drawback is that it requires a considerable amount of pre-handshake processing and requires the client and server to exchange the public portion of the generated symmetric key to encrypt and decrypt SNI. This requirement raises the security issues that need mitigation using persistent security credential modifications. %Moreover, server issues associated with ESNI lead to emergence of Encrypted Clienthello enhancements. This enhancement proposes to encrypt entire clienthello handshake message. The ECH feature is still in proposal state \cite{ech_ietf_draft}.

\item {\bf TLS 1.3 auto-downgrade}
\begin{figure}[!ht]
	\centerline{\includegraphics[scale=.085]{Figs/tls13_fallback.png}}
	\caption{Downgrading TLS 1.3 handshake message to lower TLS version}
	\label{fig:tls13_fallback}
\end{figure}
As of now, many Internet browsers support TLS 1.3. However, the working of TLS 1.3 protocol in live environment shows the downgrade of TLS handshake messages to lower version of TLS such as TLS 1.2 as shown in Fig.~\ref{fig:tls13_fallback}. It shows the downgrade of Amazon prime video-specific secure channel from TLS 1.3 to TLS 1.2 in Chromium browser (Version 96). \cite{chrome_tls13_downgrade_status} describes the issue as a results of not enabling the anti-downgrade feature \cite{chrome_tls13_downgrade} in Chrome browser due to bugs in some man-in-the-middle proxies. Such issues in the end-to-end working of TLS 1.3 protocol prevent the use of ESNI and subsequent masking of server host identity.
\end{itemize}

Such issues with the TLS 1.3 prevents the full-scale of adoption of it.
